Unfolding overlapped slitless imaging spectrometer data for extended sources

Slitless spectrometers can provide simultaneous imaging and spectral data over an extended field of view, thereby allowing rapid data acquisition for extended sources. In some instances, when the object is greatly extended or the spectral dispersion is too small, there may be locations in the focal plane where contributions from emission lines at different wavelengths contribute. It is then desirable to unfold the overlapped regions in order to isolate the contributions from the individual wavelengths. In this paper, we describe a method for such an unfolding, using an inversion technique developed for an extreme ultraviolet imaging spectrometer and coronagraph named the COronal Spectroscopic Imager in the EUV (COSIE). The COSIE spectrometer wavelength range (18.6 - 20.5 nm) contains a number of strong coronal emission lines and several density sensitive lines. We focus on optimizing the unfolding process to retrieve emission measure maps at constant temperature, maps of spectrally pure intensity in the Fe XII and Fe XIII lines and density maps based on both Fe XII and Fe XIII diagnostics.

==> densmap_aia.tex <==
D0   &   100  &  1.8  &  954  \\  
D1   &   200  &  1.6  &  44  \\  
D2   &   300  &  1.6  &  3  \\  
D3   &   400  &  1.5  &  0  \\  
\multicolumn{3}{c}{Combined}  &  1.6  &   NA  \\  

